A survey on attention mechanisms for medical applications: are we moving towards better algorithms?

The increasing popularity of attention mechanisms in deep learning algorithms for computer vision and natural language processing made these models attractive to other research domains. In healthcare, there is a strong need for tools that may improve the routines of the clinicians and the patients. Naturally, the use of attention-based algorithms for medical applications occurred smoothly. However, being healthcare a domain that depends on high-stake decisions, the scientific community must ponder if these high-performing algorithms fit the needs of medical applications. With this motto, this paper extensively reviews the use of attention mechanisms in machine learning (including Transformers) for several medical applications. This work distinguishes itself from its predecessors by proposing a critical analysis of the claims and potentialities of attention mechanisms presented in the literature through an experimental case study on medical image classification with three different use cases. These experiments focus on the integrating process of attention mechanisms into established deep learning architectures, the analysis of their predictive power, and a visual assessment of their saliency maps generated by post-hoc explanation methods. This paper concludes with a critical analysis of the claims and potentialities presented in the literature about attention mechanisms and proposes future research lines in medical applications that may benefit from these frameworks.

==> paper_contents/plots/all_plots.tex <==
% All accuracy plots
\begin{figure}[!htb]

    \minipage{0.32\textwidth}
      \includegraphics[width=\linewidth]{paper_contents/plots/aptos/plot_APTOS2019.png}
      % \caption{A really Awesome Image}\label{fig:awesome_image1}
    \endminipage\hfill
    \minipage{0.32\textwidth}
      \includegraphics[width=\linewidth]{paper_contents/plots/isic/plot_ISIC2020.png}
      % \caption{A really Awesome Image}\label{fig:awesome_image2}
    \endminipage\hfill
    \minipage{0.32\textwidth}%
      \includegraphics[width=\linewidth]{paper_contents/plots/mimiccxr/plot_MIMIC-CXR.png}
      \caption{Predictive performance (i.e., accuracy) results of the different models on the APTOS2019, ISIC2020 and MIMIC-CXR data sets, using different percentages of training data.}\label{fig:all_plots}
    \endminipage

\end{figure}


==> paper_contents/sections/tmp.tex <==
% \subsection*{The revolution of deep learning}
% Deep Learning: https://courses.cs.duke.edu/spring20/compsci527/papers/Pouyanfar.pdf
% http://www.cs.toronto.edu/~hinton/absps/NatureDeepReview.pdf
% 


% \subsection*{The importance of machine learning interpretability}
% The high success of machine learning algorithms in several tasks has motivated their implementation in critical domains (\eg, justice, healthcare) to support the work of decision-makers (\eg, judges, medical doctors). In the medical domain, there are already proposals of deep learning algorithms that claim to achieve or surpass human-like performance~\cite{mckinney_international_2020}. However, the black box behaviour of these models does not help decision-makers to have a clear understanding of their inner-functioning, thus preventing them to diagnose errors and potential biases or deciding when and how much to rely on these models~\cite{slack2020fooling}. This lack of transparency represents an obstacle to the deployment and to the adoption of these algorithms in the medical context since it jeopardises the trust of their potential users~\cite{ribeiro2016should}. There has been a huge effort into the development of post-model strategies to explain the behaviour of black box models, however, the outputs of these algorithms are prone to subjective evaluation (\ie, different users will have different interpretations)~\cite{mittelstadt2019explaining} and may be misleading~\cite{lipton_mythos_2017}. Moreover, recent works have shown that it is possible to fool these post-model methods in the sense that an arbitrary attacker can manipulate these~\textit{explanations} for their benefit (\eg, hide discriminatory biases of a black box model)~\cite{slack2020fooling,subramanya2019fooling}. Hence, we agree that just being able to obtain explanations is not enough and that we rather need to take into account at the development stage that these methods must respect specific constraints that give them the capability of generating human-understandable explanations and make decisions based on such premises~\cite{rudin_stop_2019}.

% To facilitate trust (and increase transparency) in AI algorithms it is important to ensure~\textit{a priori} that these models are interpretable. This can only be achieved if we understand first how decisions are made in the clinical context. For instance, to produce a decision, clinicians may use examples that have similarities with the sample under analysis. Contrarily, it is also common to use examples that represent the opposite to understand the decision (\ie, counterfactual explanation)~\cite{verma2020counterfactual}. This type of prior knowledge can be integrated during the training of the models (\eg, imposing model sparsity through regularisation) or before, by building models based on cases~\cite{doshi-velez_towards_2017}. On the other hand, it is important to understand what the algorithms are already learning and to evaluate the quality of such explanations (\eg, understand if the algorithms are extracting relevant features for the clinical context). A different dimension of the application of AI in sensitive domains such as healthcare is the development of ethical and fair algorithms~\cite{chen_treating_2020}. Therefore, it is fundamental that we take into account the intrinsic variability of the data sets to produce models that can be agnostic to intrinsic biases~\cite{terhorst2020post}. This strategy is supported by the new European Union’s General Data Protection Regulation (EU-GDPR)~\cite{kaminski_right_nodate} which advises that these algorithms should be able to explain their decisions for the sake of transparency. Moreover, transparent algorithms might appropriately enhance the trust of clinical professionals in future AI systems.






% A key aspect in the machine learning revolution was the possibility to reinvent deep neural networks and to train them to solve problems of different domains, such as healthcare, law or finance~\cite{lecun_deep_2015,mohseni_multidisciplinary_2019}. According to the psychology literature, humans tend to selectively concentrate on a specific part of the information~\cite{wang2016survey}. Following this intuition, the research community recognised that in AI systems, some parts of the input data are more relevant than others (e.g., in automatic translation systems, only a subset of words is relevant)~\cite{chaudhari2019attentive}.


%  Deep learning techniques, such as convolutional neural networks (CNNs) or recurrent neural networks (RNNs), have been challenging human performance at some specific tasks such as cancer detection in biomedical imaging~\cite{mckinney_international_2020} or machine translation in natural language processing~\cite{belinkov_analysis_2019}. Moreover, deep learning methods extract patterns directly from raw data (representation learning) and discover which are the relevant ones for a specific task~\cite{lecun_deep_2015, schmidhuber_deep_2015}, while conventional machine learning methods often need to employ data processing steps (\eg, data cleaning, feature extraction and feature selection) and require previous domain knowledge on the problem~\cite{domingos_few_2012}. However, these powerful techniques also present limitations. The most pertinent one is the fact that most of these models work as black boxes (\ie, their internal logic is hidden to the user) that receive data and output results without justifying their predictions in a human-understandable way~\cite{rudin_stop_2019}.

% In healthcare, this lack of transparency leads to a deficit of trust, which may jeopardise the acceptance of these technologies by health professionals. Also, there is an inherent tension between machine learning performance (predictive accuracy) and explainability: usually, the best-performing methods (\eg, deep learning) are the least transparent, and the ones providing a clear explanation (\eg, decision trees) are less accurate~\cite{holzinger_what_2017}. Therefore, the topic of explainable artificial intelligence (XAI) appeared intending to contribute to a more transparent AI~\cite{gilpin_explaining_2019, molnar_interpretable_nodate} (Figure~\ref{fig:xai_darpa} summarises the concept of XAI according to the vision of the Defense Advanced Research Projects Agency (DARPA)\footnote{\url{https://www.darpa.mil/program/explainable-artificial-intelligence}}). Although there is no clear distinction between explainability and interpretability~\cite{lipton_mythos_2017}, one may think of these as a three-stage process: pre-, in- and post-model~\cite{doshi-velez_towards_2017}. Pre-model methods focus on understanding the data distribution before building the model, through exploratory data analysis~\cite{tukey_exploratory_1977, Varshney2012InteractiveVS}. This comprehension of the data may contribute to higher confidence with the posterior decisions that a model can provide. In-model approaches seek to integrate interpretability inside the model. To do this, one may follow different strategies: models based in rules~\cite{rivest_learning_1987}, models based in cases~\cite{kim_bayesian_nodate} and the use of regularisation techniques during training to obtain sparser or monotonic models~\cite{lecun_deep_2015, gupta_monotonic_nodate}. Finally, post-model strategies are related to a posterior analysis of the model predictions. For instance, in medical imaging, this can be done using the gradient information to identify the areas of the image that mostly contribute to the final decision~\cite{simonyan_deep_2014, smilkov_smoothgrad_2017}, inserting a perturbation and observing the prediction~\cite{fernandes_deep_2018}, inverting the representations back to the input pixel space~\cite{zeiler_visualizing_2013, dosovitskiy_inverting_2016} or connecting the representations to semantic concepts~\cite{bau_network_2017}. 

% The outstanding predictive performance of deep learning models and the generalised belief that such complex models seem to uncover ``hidden patterns'' actively contributed to the research and development of post-model methods, thus contributing to their popularity among the machine learning community. However, it is relevant to point out some of the drawbacks of exclusively investing in a post-model interpretability strategy. This was extensively explored in~\cite{rudin_stop_2019}: explanations are just an approximation to what the model computes which can be dangerous in the sense that they can be inaccurate representations of the original model in parts of the feature space~\cite{mittelstadt2019explaining}; explanations may not provide enough detail to understand what the black box model is doing (\eg, explanations for two opposite classes may be the same). Moreover, in applications that depend on high stakes decisions, such as healthcare, it is fundamental to assess the quality of these explanations~\cite{rudin_stop_2019, stoyanov_towards_2018}, for the sake of transparency, ethics and fairness. On the other hand, we should start investing more efforts in pre-model interpretability, since understanding first the data distribution that we are dealing with will contribute to an increase of confidence with the posterior decisions and explanations that a given machine learning model is capable of providing~\cite{silva_how_2019}; and in in-model interpretability, since models that are inherently interpretable provide their explanations and are faithful to what the machine learning model actually computes~\cite{rudin_stop_2019}.

==> paper_contents/tables/aptos_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the APTOS2019 data set.}
\label{tab:aptos-acc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 1,000 & 0,982 & 0,976 & 194 \\
ResNet-50        & 0,998 & 0,977 & 0,980 & 60  \\
SEDenseNet-121   & 0,970 & 0,933 & 0,933 & 132 \\
SEResNet-50      & 0,999 & 0,982 & 0,982 & 91  \\
CBAMDenseNet-121 & 0,976 & 0,949 & 0,935 & 167 \\
CBAMResNet-50    & 0,965 & 0,924 & 0,931 & 157 \\
DeiT             & 0,996 & 0,981 & 0,976 & 169 \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/aptos_acc_10perc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the APTOS2019 data set on the low training data regimen, using $10\%$ of the training data.}
\label{tab:aptos-acc-10perc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 1,000 & 0,958 & 0,955 & 260 \\
ResNet-50        & 1,000 & 0,965 & 0,958 & 246 \\
SEDenseNet-121   & 0,974 & 0,909 & 0,896 & 285 \\
SEResNet-50      & 1,000 & 0,974 & 0,962 & 299 \\
CBAMDenseNet-121 & 0,979 & 0,906 & 0,880 & 290 \\
CBAMResNet-50    & 0,936 & 0,895 & 0,882 & 291 \\
DeiT             & 1,000 & 0,947 & 0,949 & 218 \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/aptos_acc_1perc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the APTOS2019 data set on the low training data regimen, using $1\%$ of the training data.}
\label{tab:aptos-acc-1perc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 1,000 & 0,859 & 0,882 & 287 \\
ResNet-50        & 1,000 & 0,907 & 0,924 & 299 \\
SEDenseNet-121   & 1,000 & 0,819 & 0,816 & 299 \\
SEResNet-50      & 1,000 & 0,886 & 0,907 & 299 \\
CBAMDenseNet-121 & 1,000 & 0,788 & 0,765 & 296 \\
CBAMResNet-50    & 0,913 & 0,754 & 0,751 & 299 \\
DeiT             & 0,957 & 0,860 & 0,878 & 280 \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/aptos_acc_50perc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the APTOS2019 data set on the low training data regimen, using $50\%$ of the training data.}
\label{tab:aptos-acc-50perc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 1,000 & 0,976 & 0,976 & 185 \\
ResNet-50        & 0,998 & 0,970 & 0,971 & 81  \\
SEDenseNet-121   & 0,973 & 0,932 & 0,918 & 184 \\
SEResNet-50      & 0,999 & 0,982 & 0,971 & 141 \\
CBAMDenseNet-121 & 0,984 & 0,945 & 0,925 & 248 \\
CBAMResNet-50    & 0,967 & 0,932 & 0,909 & 238 \\
DeiT             & 0,993 & 0,979 & 0,975 & 124 \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/isic_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the ISIC2020 data set.}
\label{tab:isic-acc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 0,998 & 0,975 & 0,974 & 162 \\
ResNet-50        & 0,993 & 0,966 & 0,964 & 101 \\
SEDenseNet-121   & 0,965 & 0,934 & 0,937 & 273 \\
SEResNet-50      & 0,995 & 0,969 & 0,969 & 140 \\
CBAMDenseNet-121 & 0,946 & 0,917 & 0,917 & 280 \\
CBAMResNet-50    & 0,900 & 0,871 & 0,879 & 298 \\
DeiT             & 0,991 & 0,966 & 0,966 & 117 \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/isic_acc_10perc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the ISIC2020 data set on the low training data regimen, using $10\%$ of the training data.}
\label{tab:isic-acc-10perc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 0,997 & 0,967 & 0,964 & 234 \\
ResNet-50        & 0,999 & 0,970 & 0,971 & 181 \\
SEDenseNet-121   & 0,967 & 0,922 & 0,927 & 283 \\
SEResNet-50      & 0,999 & 0,973 & 0,971 & 203 \\
CBAMDenseNet-121 & 0,962 & 0,918 & 0,928 & 282 \\
CBAMResNet-50    & 0,873 & 0,838 & 0,837 & 289 \\
DeiT             & 0,996 & 0,971 & 0,966 & 147 \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/isic_acc_1perc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the ISIC2020 data set on the low training data regimen, using $1\%$ of the training data.}
\label{tab:isic-acc-1perc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 0,979 & 0,954 & 0,957 & 289 \\
ResNet-50        & 1,000 & 0,974 & 0,972 & 295 \\
SEDenseNet-121   & 0,985 & 0,960 & 0,959 & 285 \\
SEResNet-50      & 1,000 & 0,968 & 0,969 & 295 \\
CBAMDenseNet-121 & 0,985 & 0,940 & 0,940 & 298 \\
CBAMResNet-50    & 0,821 & 0,814 & 0,805 & 295 \\
DeiT             & 1,000 & 0,977 & 0,974 & 299 \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/isic_acc_50perc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the ISIC2020 data set on the low training data regimen, using $50\%$ of the training data.}
\label{tab:isic-acc-50perc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 0,993 & 0,965 & 0,966 & 145 \\
ResNet-50        & 0,997 & 0,968 & 0,966 & 124 \\
SEDenseNet-121   & 0,975 & 0,937 & 0,940 & 283 \\
SEResNet-50      & 0,998 & 0,973 & 0,972 & 237 \\
CBAMDenseNet-121 & 0,953 & 0,924 & 0,927 & 299 \\
CBAMResNet-50    & 0,912 & 0,877 & 0,880 & 269 \\
DeiT             & 0,993 & 0,969 & 0,965 & 125 \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/mimiccxr_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the MIMIC-CXR data set.}
\label{tab:mimiccxr-acc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 0,877 & 0,858 & 0,846 & 58  \\
ResNet-50        & 0,873 & 0,858 & 0,862 & 27  \\
SEDenseNet-121   & 0,861 & 0,841 & 0,834 & 273 \\
SEResNet-50      & 0,886 & 0,882 & 0,834 & 48  \\
CBAMDenseNet-121 & 0,854 & 0,841 & 0,833 & 266 \\
CBAMResNet-50    & 0,806 & 0,856 & 0,825 & 220 \\
DeiT             & 0,878 & 0,856 & 0,845 & 60  \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/mimiccxr_acc_10perc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the MIMIC-CXR data set on the low training data regimen, using $10\%$ of the training data.}
\label{tab:mimiccxr-acc-10perc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 0,860 & 0,826 & 0,802 & 60 \\
ResNet-50        & 0,897 & 0,863 & 0,831 & 53  \\
SEDenseNet-121   & 0,802 & 0,796 & 0,798 & 139 \\
SEResNet-50      & 0,862 & 0,861 & 0,820 & 44  \\
CBAMDenseNet-121 & 0,811 & 0,798 & 0,779 & 283 \\
CBAMResNet-50    & 0,731 & 0,738 & 0,737 & 271 \\
DeiT             & 0,877 & 0,848 & 0,837 & 78  \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/mimiccxr_acc_1perc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the MIMIC-CXR data set on the low training data regimen, using $1\%$ of the training data.}
\label{tab:mimiccxr-acc-1perc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 0,931 & 0,800 & 0,801 & 182 \\
ResNet-50        & 0,944 & 0,816 & 0,804 & 82  \\
SEDenseNet-121   & 0,830 & 0,740 & 0,756 & 284 \\
SEResNet-50      & 0,920 & 0,820 & 0,806 & 104 \\
CBAMDenseNet-121 & 0,784 & 0,736 & 0,715 & 253 \\
CBAMResNet-50    & 0,737 & 0,717 & 0,715 & 276 \\
DeiT             & 0,850 & 0,824 & 0,787 & 60  \\ \bottomrule
\end{tabular}%
}
\end{table*}


==> paper_contents/tables/mimiccxr_acc_50perc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Predictive performance results (i.e., accuracy) obtained for the MIMIC-CXR data set on the low training data regimen, using $50\%$ of the training data.}
\label{tab:mimiccxr-acc-50perc}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Accuracy (Train)} & \textbf{Accuracy (Validation)} & \textbf{Accuracy (Test)} & \multicolumn{1}{l}{\textbf{Best Val Loss (Epoch)}} \\ \midrule
DenseNet-121     & 0,892 & 0,867 & 0,840 & 75 \\
ResNet-50        & 0,878 & 0,867 & 0,847 & 31  \\
SEDenseNet-121   & 0,831 & 0,816 & 0,814 & 157 \\
SEResNet-50      & 0,873 & 0,871 & 0,844 & 41  \\
CBAMDenseNet-121 & 0,847 & 0,822 & 0,826 & 293 \\
CBAMResNet-50    & 0,765 & 0,788 & 0,787 & 224 \\
DeiT             & 0,874 & 0,858 & 0,834 & 63  \\ \bottomrule
\end{tabular}%
}
\end{table*}

